Reliability Assessment for Distribution Systems with Embedded Microgrids

The electrical distribution system is moving toward a more decentralized, complex, and dynamic system. The system is experiencing a higher penetration of distributed energy resources, flexible resources, and active end-users, leading to an active distribution system. If these components are used actively, they can have a positive effect on the distribution system's reliability. This paper aims to investigate how a microgrid with renewable energy sources and energy storage might influence the reliability of electricity supply in a radially operated distribution system. The reliability is investigated from both the distribution system and the microgrid perspective with the application of different scenarios. The study includes an extensive sensitivity analysis. In this study, we use our developed reliability assessment tool for distribution networks. The tool is an open available software where the example network and datasets are embedded. The reliability assessment tool is based on Monte Carlo simulations where load flow calculations are included to capture the behavior of the system and system components. In this paper, the reliability tool is extended to include microgrids and microgrid controller opportunities that handle interaction strategies with the distribution network. The model is demonstrated on the IEEE 33-bus network. The result is confirmed through statistical testing showing the statistical significance of providing support from the microgrid on the distribution system's reliability.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> Sections/LoafFlow.tex <==
\subsection{Load flow and load shedding optimization problem}

% A littlebit about radial load flow and the minimiziation problem for minimizing the shedded load in the network. 

To calculate the electrical consequence of a failure in the network when there are generation resources available, a load flow calculation needs to be performed. Since the network is radially operated, a Forward-Backward sweep (FBS) approach is used to perform the load flow calculation \cite{LoadFlow, haque1996load}. The FBS approach is implemented as a load flow solver in RELSAD. The benefit of using an FBS approach is that the load flow components are calculated iteratively and do not need to go through the Jacobian matrix, as in the Newton-Raphson method. This way convergence problems arising from an ill conditioned matrix of weak networks can be avoided.  %which for some weak networks can cause an ill-conditioned matrix resulting in converges problems. 

The FBS approach updates the load flow through the backward sweep before the buses voltage magnitude and angle are updated in the forward sweep. The method is based on \cite{Olav}. 

\subsubsection*{\bf Backward sweep}
In the backward sweep, the active and reactive power over the lines is calculated. The active and reactive power over line \textit{l} for iteration \textit{k}, $P_{l}$ and $Q_{l}$, is calculated by adding the accumulated active and reactive load, $P_{l}^{'}$ and $Q_{l}^{'}$, at the downstream buses and the accumulated active and reactive power losses, $P_{l}^{*}$ and $Q_{l}^{*}$, over the downstream lines including the power loss over line $l$ and the load at the current bus %This can be seen in eq. \ref{eq:PowerA} and \ref{eq:PowerQ}

\begin{equation}
    \label{eq:PowerA}
    P_{l} = P_{l}^{'} + P_{l}^{*}
\end{equation}
\begin{equation}
    \label{eq:PowerQ}
    Q_{l} = Q_{l}^{'} + Q_{l}^{*}
\end{equation}

where the accumulated active and reactive load at the buses are calculated as 
%in eq. \ref{eq:acc_P_load} and \ref{eq:acc_Q_load}. 


\begin{equation}
    \label{eq:acc_P_load}
    P_{l}^{'} = P_{i}^{load} + \sum_{d_b} P_{d_b}^{load}
\end{equation}
\begin{equation}
    \label{eq:acc_Q_load}
    Q_{l}^{'} = Q_{i}^{load} + \sum_{d_b} Q_{d_b}^{load}
\end{equation}

Here $P_{i}^{load}$ is the active load at node $i$, $Q_{i}^{load}$ is the reactive load at node $i$, and $P_{d_{b}}^{load}$ and $Q_{d_{b}}^{load}$ are the active and reactive loads at the downstream buses, respectively. 


The accumulated active and reactive power losses are calculated as 
%in eq. \ref{eq:acc_P_loss} and \ref{eq:acc_Q_loss}. 


\begin{equation}
    \label{eq:acc_P_loss}
    P_{l}^{*} = P_{l}^{loss} + \sum_{d_l} P_{d_l}^{loss}
\end{equation}
\begin{equation}
    \label{eq:acc_Q_loss}
    Q_{l}^{*} = Q_{l}^{loss} + \sum_{d_l} Q_{d_l}^{loss}
\end{equation}

Here $P_{l}^{loss}$ and $Q_{l}^{loss}$ are the active and reactive power loss over line $l$, respectively, and $P_{d_l}^{loss}$ and $Q_{d_l}^{loss}$ are the active and reactive power loss of the downstream lines, respectively. 

The active and reactive power loss over a line is further calculated as 
%as in eq. \ref{eq:P_loss} and \ref{eq:Q_loss}.
\begin{equation}
    \label{eq:P_loss}
    P_{l}^{loss} = R_{l}\frac{P_{l}^{'2}+Q_{l}^{'2}}{V_{j}^{2}}
\end{equation}
\begin{equation}
    \label{eq:Q_loss}
    Q_{l}^{loss} = X_{l}\frac{P_{l}^{'2}+Q_{l}^{'2}}{V_{j}^{2}}
\end{equation}

Where $R_{l}$ and $X_{l}$ are the line resistance and reactance, respectively, and $V_{j}$ is the voltage at the ending bus. 



\subsubsection*{\bf Forward sweep}
In the forward sweep, the bus voltage magnitudes and angles are updated by using the updated active and reactive power from the backward sweep. Then the voltage magnitude at bus \textit{i} in relation to the voltage magnitude at bus \textit{j} for iteration \textit{k} can be calculated by

\begin{equation}
    \begin{split}
    \label{eq:Vol_magnitude}
    V_{i} &= V_{j} - I_{l}(R_{l}+jX_{l}) = \\ 
    &\sqrt{V_{j}^{2} - T_{1} + T_{2}}
    \end{split}
\end{equation}

where the terms $T_{1}$ and $T_{2}$ are 

\begin{equation*}
    T_{1} = 2(P_{l}R_{l} + Q_{l}X_{l})
\end{equation*}
\begin{equation*}
    T_{2} = \frac{(P_{l}^{2}+Q_{l}^{2})(R_{l}^{2}+X_{l}^{2})}{V_{j}^{2}}
\end{equation*}

The voltage angle can be updated as 

\begin{equation}
    \label{eq:Vol_angel}
    \delta_{i} = \delta_{j} + \arctan{\frac{Im(V_{i})}{Re(V_{i})}}    
\end{equation}

where $\delta_{j}$ is the voltage angle of bus $j$, $Im(V_{i})$ is the imaginary part of $V_{i}$, and $Re(V_{i})$ is the real part of $V_{i}$.



\begin{comment}
\begin{enumerate}
    \item Initilizing
\begin{equation}
    \label{eq:Init}
    {\tt SAIFI} = \frac{\sum_{\forall i} \lambda_{i}N_{i}}{\sum N_{i}}
\end{equation}
where $N_{i}$ is the {\em total number of customers served}, and $\sum_{\forall i} \lambda_{i}N_{i}$ is the {\em total number of customer interruptions}. ${\tt SAIFI}$ is a measure of the frequency of interruptions the customers in the system expect to experience. 
\item Backward sweep: 
In the backward sweep the active and reactive power over the lines are calculated. The active and reactive power over line \textit{l} for iteration \textit{k} is 
\begin{equation}
    \label{eq:PowerA}
    P_{l} = P_{l}^{'} + P_{l}^{*}
\end{equation}
\begin{equation}
    \label{eq:PowerQ}
    Q_{l} = Q_{l}^{'} + Q_{l}^{*}
\end{equation}

where
\begin{equation}
    P_{l}^{'} = P_{i}^{load} + \sum_{d_b} P_{d_b}^{load}
\end{equation}
\begin{equation}
    Q_{l}^{'} = Q_{i}^{load} + \sum_{d_b} Q_{d_b}^{load}
\end{equation}
\begin{equation}
    P_{l}^{*} = P_{l}^{loss} + \sum_{d_l} P_{d_l}^{loss}
\end{equation}
\begin{equation}
    Q_{l}^{*} = Q_{l}^{loss} + \sum_{d_l} Q_{d_l}^{loss}
\end{equation}

Where $P_{i}^{load}$ and $Q_{i}^{load}$ is the active and reactive load of the parent bus

and 

\begin{equation}
    P_{l}^{loss} = R_{l}\frac{P_{l}^{'2}+Q_{l}^{'2}}{V_{j}^{2}}
\end{equation}
\begin{equation}
    Q_{l}^{loss} = X_{l}\frac{P_{l}^{'2}+Q_{l}^{'2}}{V_{j}^{2}}
\end{equation}
where $\sum_{\forall i} U_{i}N_{i}$ is {\em total number of customer interruption} durations. ${\tt SAIDI}$ is a measure of the expected duration of interruptions a customer is expected to experience. 
\item Forward sweep: 
In the forward sweep the systems bus voltages are updated by using the updated active and reactive power from the backward sweep. Then the voltage magnitude at bus \textit{i} in relation to the voltage magnitude at bus \textit{j} for iteration \textit{k} is 
\begin{equation}
    \begin{split}
    \label{eq:Voltage}
    V_{i} &= V_{j} - I_{l}(R_{l}+jX_{l}) = \\ 
    &\sqrt{V_{j}^{2} - T_{1} + T_{2}}
    \end{split}
\end{equation}
\begin{equation*}
    T_{1} = 2(P_{l}R_{l} + Q_{l}X_{l})
\end{equation*}
\begin{equation*}
    T_{2} = \frac{(P_{l}^{2}+Q_{l}^{2})(R_{l}^{2}+X_{l}^{2})}{V_{j}^{2}}
\end{equation*}
 
\end{enumerate}
\end{comment}


\subsubsection*{\bf Load shedding optimization problem}
Since the system lines and the generation resources have limited capacity, a simple load shedding optimization problem is introduced in RELSAD %as seen in eq. \ref{eq:min}, is performed 
to minimize the total shedded load in the network based on the price. The price is based on the \textit{Cost of energy not supplied} (CENS) \cite{KILENVE}. The CENS scheme, in Norway, is intended to give the DSOs incentive to build and operate the network with a focus on a socio-economic and reliable operation. Similar schemes can be seen in \cite{chowdhury2001application, sullivan1996interruption}. However, a more advanced optimization problem could be implemented but this is not the scope of this study. %The KILE cost represents the customer's costs during an interruption in power and the costs are calculated for different customer groups. 

The load shedding optimization problem, in eq. \ref{eq:min}, minimizes the total load shedded in the network based on the CENS for shedding that specific load type. This is subjected to load flow balance and capacity limitations over the power lines, the load, and the generation. Here $C_n$ is the cost of shedding load at node n while $P_{n}^{s}$ is the amount of shedded power at node n. $P_{j}^{g}$ is the production from generator $j$. $P_{k}^{d}$ is the load demand at node $k$ while $P_{i}^{l}$ is the power transferred over line $i$. $\gamma_i$ = 1 if line $i$ is the starting point, -1 if line $i$ is the ending point. $\lambda_j$ = 1 if there is a production unit at node $j$, otherwise it is 0. $\mu_k$ = 1 if there is a load on node $k$, otherwise it is 0.

\begin{comment}
\begin{align*}
    \underset{P_{shed,n}}{\text{minimize}}& \quad P_{shed, tot} = \sum_{n = 1}^{N_n}   C_{n}\cdot P_{shed,n}\\
    \text{s.t.} &\\
    & \begin{aligned}
        \sum_{l = 1}^{N_l} \gamma_l \cdot P_{line, l} &= \sum_{g = 1}^{N_g} \lambda_g \cdot P_{gen, g} - \sum_{n = 1}^{N_n} \mu_n \cdot P_{load, n}\\
        &+ \sum_{n = 1}^{N_n} \mu_n \cdot P_{shed, n}
    \end{aligned} \\
    &\begin{aligned}
        P_{gen, g}^{min} &\leq& P_{gen, g} &\leq& P_{gen, g}^{max} \\
        0 &\leq& P_{shed, n} &\leq& P_{load, n} \\
        -P_{line, l}^{max} &\leq& P_{line, l} &\leq& P_{line, l}^{max}       
    \end{aligned}
\end{align*}
\end{comment}

\begin{align}
    &\underset{P^{s}_{n}}{\text{minimize}}
    \quad \mathcal{P}_s = \sum_{n = 1}^{N_n}   C_{n}\cdot P^{s}_{n} \label{eq:min}\\
    &\text{subject to: } \nonumber \\
    &\begin{aligned}
        \sum_{i=1}^{N_l} \gamma_i \cdot P^{l}_{i} &= \sum_{j=1}^{N_g} \lambda_j \cdot P^{g}_{j} - \sum_{k = 1}^{N_n}& \mu_k& \cdot (P^{d}_{k} - P^{s}_{k})\\
        \min P_{j}^{g} &\leq P_{j}^{g} \leq \max P_{j}^{g} &\forall j&=1,\dots,N_{g}\\
        0 &\leq P_{k}^{s} \leq P_{k}^{d}  &\forall k&=1,\dots,N_{n}\\
        \left| P_{i}^{l} \right| &\leq \max P_{i}^{l}  &\forall i&=1,\dots,N_{l}\\
    \end{aligned} \nonumber
\end{align}


==> Sections/RELSAD_description.tex <==
\subsection{Description of RELSAD}

RELSAD is based on RELRAD -- an analytical approach for distribution system reliability assessment. RELRAD is an example of an analytical approach developed for calculating the reliability in a radial operated distribution system \cite{RELRAD}. The RELRAD methodology calculates the individual load point reliability indices analytically based on the fault contribution from all the network components and their consequence on a given load point. However, such an approach does not consider the active components in the network, such as microgrids, DG, and batteries, and since it uses average values for load and generation, the electrical consequence and the behavior of the network are not considered. Therefore, simulation is a more suitable method to calculate the reliability in an active distribution system including microgrids, flexible resources, and DG.  

RELSAD however, is a tool developed for assessing the reliability of modern distribution systems. RELSAD is a general tool that can consider any network that operates radially. In RELSAD, a power system - $P_{s}$ is first created before distribution systems - $D_{s}$ and microgrids - $M_{s}$ are created inside the $P_{s}$. After this, the electrical system components can be created and added to associated network layers. The electrical components are lines - $l$, buses - $b$, disconnectors - $d$, circuit breakers - $cb$, generation units - $p_{u}$, and batteries - $p_{b}$. In addition, a load - $p_{d}$ can be assigned to each bus. 

The incremental procedure of the failure handling model is illustrated in Algorithm \ref{alg:procedure}. After a $P_{s}$ is created with associated systems and components, the incremental procedure will set the load and generation at the system buses for the current time increment. Then the failure status of each component is drawn based on random sampling and the failure rate of the different components. If any component is in a failed state, the $D_{s}$ and/or $M_{s}$ with the failed components will be divided into sub-systems, and a load flow and load shedding optimization problem will be solved for each sub-system. The load flow and load shedding optimization problem are included to calculate the electrical consequence of a failure when active components are present. When this is performed, the historical variables of the components are updated. The historical variables can then further be used to evaluate the reliability of the $P_{s}$, the different subnetworks (the $D_{s}$ and $M_{s}$), and the individual load points. 
The rest of this section aims to describe the different procedures of the reliability evaluation in greater detail. 

%First, the system is initialized and the parameters set. Then the algorithm will check for failures in the system. If there are any failures, the system will be divided into sub-systems and a load flow and minimization problem will be solved for each sub-system. 
%This paper does not consider a true Monte Carlo simulation since it uses the element of time and will therefore not simulate a fully random process. 

\begin{algorithm}
    \SetAlgoLined
     Set bus $p_d$ and $p_u$ for the current time increment\;
     Draw component fail status\;
     \If{Failure in $P_s$ (in the systems, $D_s$ and $M_s$)}{
         Find sub-systems\;
         \ForEach{sub-system}{
            Update $p_b$ demand (charge or discharge rate)\;
            Run load flow\;
            Run load shedding optimization problem\;
         }
         Update history variables\;
     }
    \caption{Increment procedure}
    \label{alg:procedure}
\end{algorithm}


%To consider the function of the system, the state of the system at the simulated time-step needs to be calculated. This can be done through load flow calculation. By adding load flow calculation into the simulation, the condition and behavior of the system can be calculated at all the wanted time-steps. In addition, the behavior of the battery and the DGs will, therefore, also be included and considered and the impact from the resources in the microgrid can be calculated more accurately. The electrical consequence of a failure can be calculated and varied load and production can be simulated. 

% Legge inn at man må klare å modellere disse nye komponentene, hvordan skal det gjøres? 

%In addition, it is important to be aware of the condition in the system at all time and the behavior of the network needs to be available. Therefore, load flow calculation needs to be added in the reliability assessment in order to get the behavior of the network and get the electrical consequences of different situations in the system. 
